Parallel parametric linear programming solving, and application to polyhedral computations

Parametric linear programming is central in polyhedral computations and in certain control applications.We propose a task-based scheme for parallelizing it, with quasi-linear speedup over large problems.

==> conclu.tex <==
\section{Conclusion and future work}
\label{sec:conclu}
We have successfully parallelized computations over convex polyhedra represented as constraints, most importantly parametric linear programming.
Speedups are particularly satisfactory for the most complex cases: polyhedra with many constraints in higher dimension.

The main cause of inefficiency in our current implementation is geometrical degeneracy, which causes overlapping regions.
Several approaches are being studied in this respect, all based on enforcing that, for given parameters, there should be only one optimal basis.%
%\footnote{For some of our applications, such as polyhedral projection, there cannot be several optimal vertices for the same parameters, except at region boundaries, so that source of degeneracy is not present. There however remains the other source, that is, several bases for the same vertex.}

The floating-point simplex algorithm is restarted from scratch in each task.
It could be more efficient to store in the task structure the last basis used, or even the full simplex tableau, to start solving from that basis instead of the default initial.
The intuition is that neighboring regions are likely to have similar bases.

The check whether a vector belongs to an already processed region, is currently implemented very simplistic: the vector is searched for in every region.
A binary space partitioning region storage could be used instead.
%: build a tree with nodes adorned by hyperplanes, all regions wholly on one side of the hyperplane under the first child, all regions wholly on the other side under the second child, all regions straddling the hyperplane in both branches, and so recursively in the branches.
%Then a region covering a vector is searched for by testing, at each node, on which side of the hyperplane the vector lies, and entering the branch.
%An appropriate locking scheme would however have to be designed.

Our coarse-grained parallelism for parametric linear programming is highly dependent on the geometry of the problem.
If there are too few regions, there are too few tasks to keep the cores busy.
One could use two levels of parallelism, with parallel linear programming, parallel exact reconstruction, etc. in each task.,
using parallel matrix computations.
%One possibility would be to parallelize floating-point linear programming and exact matrix computations,
%both handled by external libraries.
%These phases are based on matrix operations (either floating-point, rational, or integer modular), so the usual parallelization schemes for matrix computations should apply.
%One should keep in mind, however, that our matrices are much smaller than the ones typically used in high performance computing applications.
%One option could be to replace GLPK by another library based on BLAS, such as Coin-OR LP, and use a parallel BLAS implementation such as Goto-BLAS or Intel MKL.
%With respect to Flint, we attempted to run certain internal matrix computation loops in parallel, but gave up due to crashes; perhaps this could be done with more careful examination of shared data structures or the collaboration of the library maintainer.

% While our approach based on (in)equalities only does not blow up exponentially when the polyhedron is a Cartesian product of simple polyhedra, as opposed to the double description, it would likely benefit from being applied separately to terms of a Cartesian product as opposed to over the full product, perhaps in parallel.
% %some computations are performed over dense matrices, and, even if sparseness is exploited, it is easier to exploit it at a coarse level.
% We think of combining our approach with a Cartesian decomposition
% \cite{DBLP:journals/fmsd/HalbwachsMG06}.

%%% Local Variables:
%%% ispell-local-dictionary: "en"
%%% TeX-master: "main"
%%% End:

